Calibration System and Algorithm Design for a Soft Hinged Micro Scanning Mirror with a Triaxial Hall Effect Sensor

Micro scanning mirrors (MSM) extend the range and field of view of LiDARs, medical imaging devices, and laser projectors. However, a new class of soft-hinged MSMs contains out-of-plane translation in addition to the 2 degree-of-freedom rotations, which presents a cabliration challenge. We report a new calibration system and algorithm design to address the challenge. In the calibration system, a new low-cost calibration rig design employs a minimal 2-laser beam approach. The new new algorithm builds on the reflection principle and an optimization approach to precisely measure MSM poses. To establish the mapping between Hall sensor readings and MSM poses, we propose a self-synchronizing periodicity-based model fitting calibration approach. We achieve an MSM poses estimation accuracy of 0.020{\deg} with a standard deviation of 0.011{\deg}.

==> Makefile <==
all: bib
	make pdf
	make pdf
	mv root.pdf MirrorCalibration.pdf
	cp MirrorCalibration.pdf ../RAL_Review/Response-To-Review-Letter/
	#cp ../MirrorCalibration.pdf ../RAL_Review/Response-To-Review-Letter/MirrorCalibration-1.pdf
	lualatex -synctex=1 -interaction=nonstopmode ../RAL_Review/Response-To-Review-Letter/main
bib: pdf
	bibtool -- 'add.field{hreftitle="\href{%s(url)}{%s(title)}"}' bib/di-org.bib -o bib/di.bib
	bibtool -- 'delete.field{url}' bib/di.bib -o bib/di.bib
	bibtool -- 'delete.field{title}' bib/di.bib -o bib/di.bib
	bibtool -- 'rename.field{hreftitle=title}' bib/di.bib -o bib/di.bib
	bibtex root
pdf:
	-pdflatex -synctex=1 -interaction=nonstopmode root
clean:
	rm *.aux *.log *.out *.bbl *.blg *.bcf *.xml *.gz

